Vashantor: A Large-scale Multilingual Benchmark Dataset for Automated Translation of Bangla Regional Dialects to Bangla Language

The Bangla linguistic variety is a fascinating mix of regional dialects that contributes to the cultural diversity of the Bangla-speaking community. Despite extensive study into translating Bangla to English, English to Bangla, and Banglish to Bangla in the past, there has been a noticeable gap in translating Bangla regional dialects into standard Bangla. In this study, we set out to fill this gap by creating a collection of 32,500 sentences, encompassing Bangla, Banglish, and English, representing five regional Bangla dialects. Our aim is to translate these regional dialects into standard Bangla and detect regions accurately. To tackle the translation and region detection tasks, we propose two novel models: DialectBanglaT5 for translating regional dialects into standard Bangla and DialectBanglaBERT for identifying the dialect's region of origin. DialectBanglaT5 demonstrates superior performance across all dialects, achieving the highest BLEU score of 71.93, METEOR of 0.8503, and the lowest WER of 0.1470 and CER of 0.0791 on the Mymensingh dialect. It also achieves strong ROUGE scores across all dialects, indicating both accuracy and fluency in capturing dialectal nuances. In parallel, DialectBanglaBERT achieves an overall region classification accuracy of 89.02%, with notable F1-scores of 0.9241 for Chittagong and 0.8736 for Mymensingh, confirming its effectiveness in handling regional linguistic variation. This is the first large-scale investigation focused on Bangla regional dialect translation and region detection. Our proposed models highlight the potential of dialect-specific modeling and set a new benchmark for future research in low-resource and dialect-rich language settings.

==> Reference2.tex <==
@article{tong2amp,
  title={\&amp; Koller, D.(2001). Support vector machine active learning with applications to text classification},
  author={Tong, S},
  journal={Journal of Machine Learning Research},
  volume={2}
}

@article{tenenboim2008ontology,
  title={Ontology-based classification of news in an electronic newspaper},
  author={Tenenboim, Lena and Shapira, Bracha and Shoval, Peretz},
  year={2008},
  publisher={Institute of Information Theories and Applications FOI ITHEA}
}

@article{pendharkar2007topic,
  title={Topic categorization of rss news feeds},
  author={Pendharkar, Bhushan and Ambekar, Pooja and Godbole, Prajakta and Joshi, Sanket and Abhyankar, Srushti},
  journal={Group},
  volume={4},
  pages={1},
  year={2007},
  publisher={Citeseer}
}

@inproceedings{carreira2004evaluating,
  title={Evaluating adaptive user profiles for news classification},
  author={Carreira, Ricardo and Crato, Jaime M and Gon{\c{c}}alves, Daniel and Jorge, Joaquim A},
  booktitle={Proceedings of the 9th international conference on Intelligent user interfaces},
  pages={206--212},
  year={2004}
}

@article{fauzi2016indonesian,
  title={Indonesian news classification using Na{\"\i}ve Bayes and two-phase feature selection model},
  author={Fauzi, M Ali and Arifin, Agus Zainal and Gosaria, Sonny Christiano and Prabowo, Isnan Suryo},
  journal={Indonesian Journal of Electrical Engineering and Computer Science},
  volume={2},
  number={3},
  pages={401--408},
  year={2016}
}

@inproceedings{chy2014bangla,
  title={Bangla news classification using naive Bayes classifier},
  author={Chy, Abu Nowshed and Seddiqui, Md Hanif and Das, Sowmitra},
  booktitle={16th Int'l Conf. Computer and Information Technology},
  pages={366--371},
  year={2014},
  organization={IEEE}
}

@article{dutta2011machine,
  title={Machine learning approach for the classification of demonstrative pronouns for Indirect Anaphora in Hindi News Items},
  author={Dutta, Kamlesh and Kaushik, Saroj and Prakash, Nupur},
  journal={The Prague Bulletin of Mathematical Linguistics},
  volume={95},
  pages={33},
  year={2011},
  publisher={De Gruyter Poland}
}

@article{el2016arabic,
  title={Arabic news classification using field association words},
  author={El-Barbary, OG},
  journal={Advances in research},
  pages={1--9},
  year={2016}
}

@inproceedings{beresi2004automatic,
  title={Automatic classification of news articles in Spanish},
  author={Beresi, Ulises Cervino and Adeva, JJ Garc{\i}a and Calvo, Rafael A and Ceccatto, Alejandro H},
  booktitle={Actas del Congreso Argentino de Ciencias de Computaci{\'o}n (CACIC)},
  pages={1588--1600},
  year={2004}
}

@inproceedings{kabir2015bangla,
  title={Bangla text document categorization using stochastic gradient descent (sgd) classifier},
  author={Kabir, Fasihul and Siddique, Sabbir and Kotwal, Mohammed Rokibul Alam and Huda, Mohammad Nurul},
  booktitle={2015 International Conference on Cognitive Computing and Information Processing (CCIP)},
  pages={1--4},
  year={2015},
  organization={IEEE}
}

@ARTICLE{9916245,  author={Hasib, Khan Md. and Tanzim, Anika and Shin, Jungpil and Faruk, Kazi Omar and Mahmud, Jubayer Al and Mridha, M. F.},  journal={IEEE Access},   title={BMNet-5: A Novel Approach of Neural Network to Classify the Genre of Bengali Music Based on Audio Features},   year={2022},  volume={10},  number={},  pages={108545-108563},  doi={10.1109/ACCESS.2022.3213818}}

@article{yeasminmulti,
  title={Multi-category Bangla News Classification using Machine Learning Classifiers and Multi-layer Dense Neural Network},
  author={Yeasmin, Sharmin and Kuri, Ratnadip and Rana, ARM Mahamudul Hasan and Uddin, Ashraf and Pathan, AQM Sala Uddin and Riaz, Hasnat}
}

@inproceedings{selamat2003neural,
  title={Neural networks for web page classification based on augmented PCA},
  author={Selamat, Ali and Omatu, Sigeru},
  booktitle={Proceedings of the International Joint Conference on Neural Networks, 2003.},
  volume={3},
  pages={1792--1797},
  year={2003},
  organization={IEEE}
}

@article{hossain975different,
  title={Different Machine Learning based Approaches of Baseline and Deep Learning Models for Bengali News Categorization},
  author={Hossain, Mohammad Rabib and Sarkar, Soikot and Rahman, Moqsadur},
  journal={International Journal of Computer Applications},
  volume={975},
  pages={8887}
}

@inproceedings{chakraborty2019bangla,
  title={Bangla document categorisation using multilayer dense neural network with TF-IDF},
  author={Chakraborty, Manisha and Huda, Mohammad Nurul},
  booktitle={2019 1st International Conference on Advances in Science, Engineering and Robotics Technology (ICASERT)},
  pages={1--4},
  year={2019},
  organization={IEEE}
}

@article{mandal2014supervised,
  title={Supervised learning methods for bangla web document categorization},
  author={Mandal, Ashis Kumar and Sen, Rikta},
  journal={arXiv preprint arXiv:1410.2045},
  year={2014}
}

@inproceedings{harrag2009neural,
  title={Neural Network for Arabic text classification},
  author={Harrag, Fouzi and El-Qawasmah, Eyas},
  booktitle={2009 Second International Conference on the Applications of Digital Information and Web Technologies},
  pages={778--783},
  year={2009},
  organization={IEEE}
}

@article{fauzi2016indonesian,
  title={Indonesian news classification using Na{\"\i}ve Bayes and two-phase feature selection model},
  author={Fauzi, M Ali and Arifin, Agus Zainal and Gosaria, Sonny Christiano and Prabowo, Isnan Suryo},
  journal={Indonesian Journal of Electrical Engineering and Computer Science},
  volume={2},
  number={3},
  pages={401--408},
  year={2016}
}

@article{dutta2011machine,
  title={Machine learning approach for the classification of demonstrative pronouns for Indirect Anaphora in Hindi News Items},
  author={Dutta, Kamlesh and Kaushik, Saroj and Prakash, Nupur},
  journal={The Prague Bulletin of Mathematical Linguistics},
  volume={95},
  pages={33},
  year={2011},
  publisher={De Gruyter Poland}
}

@article{el2016arabic,
  title={Arabic news classification using field association words},
  author={El-Barbary, OG and others},
  journal={SCIENCEDOMAIN Int},
  volume={6},
  number={1--9},
  year={2016}
}

@inproceedings{beresi2004automatic,
  title={Automatic classification of news articles in Spanish},
  author={Beresi, Ulises Cervino and Adeva, JJ Garc{\i}a and Calvo, Rafael A and Ceccatto, Alejandro H},
  booktitle={Actas del Congreso Argentino de Ciencias de Computaci{\'o}n (CACIC)},
  pages={1588--1600},
  year={2004}
}

@inproceedings{zabir2020bangla,
  title={Bangla Newspaper Dataset},
  author={Zabir Al Nazi},
  booktitle={Kaggle},
  pages={},
  year={2020},
  doi={10.34740/KAGGLE/DSV/ 1576225}
}

@incollection{wu2020feature,
  title={Feature extraction based on improved feature weighting algorithm},
  author={Wu, ShuangXin and Jia, Ji Kang},
  booktitle={Recent Trends in Decision Science and Management},
  pages={703--708},
  year={2020},
  publisher={Springer}
}

@article{kohoutova2020toward,
  title={Toward a unified framework for interpreting machine-learning models in neuroimaging},
  author={Kohoutov{\'a}, Lada and Heo, Juyeon and Cha, Sungmin and Lee, Sungwoo and Moon, Taesup and Wager, Tor D and Woo, Choong-Wan},
  journal={Nature protocols},
  volume={15},
  number={4},
  pages={1399--1435},
  year={2020},
  publisher={Nature Publishing Group}
}


@inproceedings{han2005borderline,
  title={Borderline-SMOTE: a new over-sampling method in imbalanced data sets learning},
  author={Han, Hui and Wang, Wen-Yuan and Mao, Bing-Huan},
  booktitle={International conference on intelligent computing},
  pages={878--887},
  year={2005},
  organization={Springer}
}

@inproceedings{ribeiro2016should,
  title={Why should i trust you? Explaining the predictions of any classifier},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={Proceedings of the 22nd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={1135--1144},
  year={2016}
}

@article{atenstaedt2012word,
  title={Word cloud analysis of the BJGP},
  author={Atenstaedt, Rob},
  journal={British Journal of General Practice},
  volume={62},
  number={596},
  pages={148--148},
  year={2012},
  publisher={British Journal of General Practice}
}

@inproceedings{popel2018hybrid,
  title={A hybrid under-sampling method (HUSBoost) to classify imbalanced data},
  author={Popel, Mahmudul Hasan and Hasib, Khan Md and Habib, Syed Ahsan and Shah, Faisal Muhammad},
  booktitle={2018 21st international conference of computer and information technology (ICCIT)},
  pages={1--7},
  year={2018},
  organization={IEEE}
}

@inproceedings{ribeiro2016should,
  title={" Why should i trust you?" Explaining the predictions of any classifier},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={Proceedings of the 22nd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={1135--1144},
  year={2016}
}

@inproceedings{sazzed2019sentiment,
  title={A sentiment classification in bengali and machine translated english corpus},
  author={Sazzed, Salim and Jayarathna, Sampath},
  booktitle={2019 IEEE 20th international conference on information reuse and integration for data science (IRI)},
  pages={107--114},
  year={2019},
  organization={IEEE}
}
@inproceedings{houwelingen1992ridge,
  title={Ridge estimators in logistic regression},
  author={Houwelingen, SLC and Van, JC},
  booktitle={Royal Statistical Society},
  volume={43},
  number={1},
  pages={95--108},
  year={1992}
}

@article{pandya2014fault,
  title={Fault diagnosis of rolling element bearing by using multinomial logistic regression and wavelet packet transform},
  author={Pandya, D\_H and Upadhyay, Sanjay H and Harsha, Suraj Prakash},
  journal={Soft Computing},
  volume={18},
  number={2},
  pages={255--266},
  year={2014},
  publisher={Springer}
}

@article{gaikwad2014credit,
  title={Credit card fraud detection using decision tree induction algorithm},
  author={Gaikwad, Jyoti R and Deshmane, Amruta B and Somavanshi, Harshada V and Patil, Snehal V and Badgujar, Rinku A},
  journal={International Journal of Innovative Technology and Exploring Engineering (IJITEE)},
  volume={4},
  number={6},
  pages={66--69},
  year={2014},
  publisher={Citeseer}
}

@inproceedings{ria2020toward,
  title={Toward an enhanced bengali text classification using saint and common form},
  author={Ria, Nushrat Jahan and Khushbu, Sharun Akter and Yousuf, Mohammad Abu and Masum, Abu Kaisar Mohammad and Abujar, Sheikh and Hossain, Syed Akhter},
  booktitle={2020 11th international conference on computing, communication and networking technologies (ICCCNT)},
  pages={1--5},
  year={2020},
  organization={IEEE}
}

@article{mandal2014supervised,
  title={Supervised learning methods for Bangla web document categorization},
  author={Mandal, Ashis Kumar and Sen, Rikta},
  journal={arXiv preprint arXiv:1410.2045},
  year={2014}
}

@inproceedings{chy2014bangla,
  title={Bangla news classification using naive Bayes classifier},
  author={Chy, Abu Nowshed and Seddiqui, Md Hanif and Das, Sowmitra},
  booktitle={16th Int'l Conf. Computer and Information Technology},
  pages={366--371},
  year={2014},
  organization={IEEE}
}

@inproceedings{chakraborty2019bangla,
  title={Bangla document categorisation using multilayer dense neural network with TF-IDF},
  author={Chakraborty, Manisha and Huda, Mohammad Nurul},
  booktitle={2019 1st International Conference on Advances in Science, Engineering and Robotics Technology (ICASERT)},
  pages={1--4},
  year={2019},
  organization={IEEE}
}

@article{karim2020comparative,
  title={A Comparative Study of Different Deep Learning Model for Recognition of Handwriting Digits},
  author={Karim, Asif and Ghosh, Pronab and Anjum, Atqiya Abida and Junayed, Masum Shah and Md, Zahid Hasan and Hasib, Khan Md and Bin Emran, Al Nahian},
  year={2020},
  publisher={ICICNIS}
}

@book{rashid2016make,
  title={Make your own neural network},
  author={Rashid, Tariq},
  year={2016},
  publisher={CreateSpace Independent Publishing Platform}
}

@article{plate2000visualizing,
  title={Visualizing the function computed by a feedforward neural network},
  author={Plate, Tony A and Bert, Joel and Grace, John and Band, Pierre},
  journal={Neural computation},
  volume={12},
  number={6},
  pages={1337--1353},
  year={2000},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}

@INPROCEEDINGS{9396879,  author={Hasib, Khan Md. and Habib, Md. Ahsan and Towhid, Nurul Akter and Showrov, Md. Imran Hossain},  booktitle={2021 International Conference on Information and Communication Technology for Sustainable Development (ICICT4SD)},   title={A Novel Deep Learning based Sentiment Analysis of Twitter Data for US Airline Service},   year={2021},  volume={},  number={},  pages={450-455},  doi={10.1109/ICICT4SD50815.2021.9396879}}

@article{le2006convolutional,
  title={A convolutional neural network approach for objective video quality assessment},
  author={Le Callet, Patrick and Viard-Gaudin, Christian and Barba, Dominique},
  journal={IEEE transactions on neural networks},
  volume={17},
  number={5},
  pages={1316--1327},
  year={2006},
  publisher={IEEE}
}

@inproceedings{munikar2019fine,
  title={Fine-grained sentiment classification using bert},
  author={Munikar, Manish and Shakya, Sushil and Shrestha, Aakash},
  booktitle={2019 Artificial Intelligence for Transforming Business and Society (AITB)},
  volume={1},
  pages={1--5},
  year={2019},
  organization={IEEE}
}

@inproceedings{islam2018hand,
  title={Hand gesture feature extraction using deep convolutional neural network for recognizing American sign language},
  author={Islam, Md Rashedul and Mitu, Ummey Kulsum and Bhuiyan, Rasel Ahmed and Shin, Jungpil},
  booktitle={2018 4th International Conference on Frontiers of Signal Processing (ICFSP)},
  pages={115--119},
  year={2018},
  organization={IEEE}
}

@INPROCEEDINGS{9667818,  author={Hasib, Khan Md. and Towhid, Nurul Akter and Alam, Md. Golam Rabiul},  booktitle={2021 5th International Conference on Electrical Engineering and Information Communication Technology (ICEEICT)},   title={Online Review based Sentiment Classification on Bangladesh Airline Service using Supervised Learning},   year={2021},  volume={},  number={},  pages={1-6},  doi={10.1109/ICEEICT53905.2021.9667818}}

@INPROCEEDINGS{9720806,  author={Hasib, Khan Md. and Rahman, Farhana and Hasnat, Rashik and Alam, Md. Golam Rabiul},  booktitle={2022 IEEE 12th Annual Computing and Communication Workshop and Conference (CCWC)},   title={A Machine Learning and Explainable AI Approach for Predicting Secondary School Student Performance},   year={2022},  volume={},  number={},  pages={0399-0405},  doi={10.1109/CCWC54503.2022.9720806}}

@inproceedings{alam2021comparison,
  title={Comparison of Different CNN Model used as Encoders for Image Captioning},
  author={Alam, Md Sahrial and Rahman, Md Sayedur and Hosen, Md Ikbal and Mubin, Khairul Anam and Hossen, Sharif and Mridha, MF},
  booktitle={2021 International Conference on Data Analytics for Business and Industry (ICDABI)},
  pages={523--526},
  year={2021},
  organization={IEEE}
}

@article{zhang2015sensitivity,
  title={A sensitivity analysis of (and practitioners' guide to) convolutional neural networks for sentence classification},
  author={Zhang, Ye and Wallace, Byron},
  journal={arXiv preprint arXiv:1510.03820},
  year={2015}
}

@inproceedings{upadhyay2011enhanced,
  title={Enhanced Bangla Character Recognition using ANN},
  author={Upadhyay, Piu and Barman, Sumana and Bhattacharyya, Debnath and Dixit, Manish},
  booktitle={2011 International Conference on Communication Systems and Network Technologies},
  pages={194--197},
  year={2011},
  organization={IEEE}
}

@inproceedings{hasib2021online,
  title={Online Review based Sentiment Classification on Bangladesh Airline Service using Supervised Learning},
  author={Hasib, Khan Md and Towhid, Nurul Akter and Alam, Md Golam Rabiul},
  booktitle={2021 5th International Conference on Electrical Engineering and Information \& Communication Technology (ICEEICT)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}
@article{sennrich2015neural,
  title={Neural machine translation of rare words with subword units},
  author={Sennrich, Rico and Haddow, Barry and Birch, Alexandra},
  journal={arXiv preprint arXiv:1508.07909},
  year={2015}
}

@article{alam2020bangla,
  title={Bangla text classification using transformers},
  author={Alam, Tanvirul and Khan, Akib and Alam, Firoj},
  journal={arXiv preprint arXiv:2011.04446},
  year={2020}
}
@article{mridha2021boost,
  title={L-Boost: Identifying Offensive Texts From Social Media Post in Bengali},
  author={Mridha, MF and Wadud, Md Anwar Hussen and Hamid, Md Abdul and Monowar, Muhammad Mostafa and Abdullah-Al-Wadud, M and Alamri, Atif},
  journal={Ieee Access},
  volume={9},
  pages={164681--164699},
  year={2021},
  publisher={IEEE}
}

@article{seiffert2009rusboost,
  title={RUSBoost: A hybrid approach to alleviating class imbalance},
  author={Seiffert, Chris and Khoshgoftaar, Taghi M and Van Hulse, Jason and Napolitano, Amri},
  journal={IEEE Transactions on Systems, Man, and Cybernetics-Part A: Systems and Humans},
  volume={40},
  number={1},
  pages={185--197},
  year={2009},
  publisher={IEEE}
}
@article{hasib2020survey,
  title={A survey of methods for managing the classification and solution of data imbalance problem},
  author={Hasib, Khan Md and Iqbal, Md and Shah, Faisal Muhammad and Mahmud, Jubayer Al and Popel, Mahmudul Hasan and Showrov, Md and Hossain, Imran and Ahmed, Shakil and Rahman, Obaidur and others},
  journal={arXiv preprint arXiv:2012.11870},
  year={2020}
}

@article{shaikh2021towards,
  title={Towards improved classification accuracy on highly imbalanced text dataset using deep neural language models},
  author={Shaikh, Sarang and Daudpota, Sher Muhammad and Imran, Ali Shariq and Kastrati, Zenun},
  journal={Applied Sciences},
  volume={11},
  number={2},
  pages={869},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{jan2017sensor,
  title={Sensor fault classification based on support vector machine and statistical time-domain features},
  author={Jan, Sana Ullah and Lee, Young-Doo and Shin, Jungpil and Koo, Insoo},
  journal={IEEE Access},
  volume={5},
  pages={8682--8690},
  year={2017},
  publisher={IEEE}
}

@article{saha2014analysis,
  title={Analysis of Bangla Root Word for Universal Networking Language (UNL)},
  author={Saha, Aloke Kumar and Mridha, MF and Das, Jugal Krishna},
  journal={International Journal of Computer Applications},
  volume={89},
  number={17},
  year={2014}
}

@article{mandal2014supervised,
  title={Supervised learning methods for Bangla web document categorization},
  author={Mandal, Ashis Kumar and Sen, Rikta},
  journal={arXiv preprint arXiv:1410.2045},
  year={2014}
}

@incollection{dhar2018application,
  title={Application of tf-idf feature for categorizing documents of online bangla web text corpus},
  author={Dhar, Ankita and Dash, Niladri Sekhar and Roy, Kaushik},
  booktitle={Intelligent Engineering Informatics},
  pages={51--59},
  year={2018},
  publisher={Springer}
}

@inproceedings{al2018bangla,
  title={Bangla content categorization using text based supervised learning methods},
  author={Al Mostakim, Sadek and Ehsan, Faiza and Hasan, Syeda Mahdiea and Islam, Sadia and Shatabda, Swakkhar},
  booktitle={2018 International Conference on Bangla Speech and Language Processing (ICBSLP)},
  pages={1--6},
  year={2018},
  organization={IEEE}
}

@article{ahmed2021cyberbullying,
  title={Cyberbullying detection using deep neural network from social media comments in bangla language},
  author={Ahmed, Md Faisal and Mahmud, Zalish and Biash, Zarin Tasnim and Ryen, Ahmed Ann Noor and Hossain, Arman and Ashraf, Faisal Bin},
  journal={arXiv preprint arXiv:2106.04506},
  year={2021}
}

@inproceedings{kabir2015bangla,
  title={Bangla text document categorization using stochastic gradient descent (sgd) classifier},
  author={Kabir, Fasihul and Siddique, Sabbir and Kotwal, Mohammed Rokibul Alam and Huda, Mohammad Nurul},
  booktitle={2015 International Conference on Cognitive Computing and Information Processing (CCIP)},
  pages={1--4},
  year={2015},
  organization={IEEE}
}

@inproceedings{chakraborty2019bangla,
  title={Bangla document categorisation using multilayer dense neural network with TF-IDF},
  author={Chakraborty, Manisha and Huda, Mohammad Nurul},
  booktitle={2019 1st International Conference on Advances in Science, Engineering and Robotics Technology (ICASERT)},
  pages={1--4},
  year={2019},
  organization={IEEE}
}

@inproceedings{salehin2021comparative,
  title={A Comparative Study of Different Text Classification Approaches for Bangla News Classification},
  author={Salehin, Kamrus and Alam, M Kaosar and Nabi, Md Ashifun and Ahmed, Fahim and Ashraf, Faisal Bin},
  booktitle={2021 24th International Conference on Computer and Information Technology (ICCIT)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@inproceedings{alam2018bard,
  title={Bard: Bangla article classification using a new comprehensive dataset},
  author={Alam, Md Tanvir and Islam, Md Mofijul},
  booktitle={2018 International Conference on Bangla Speech and Language Processing (ICBSLP)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}

@inproceedings{purkaystha2018layered,
  title={Layered representation of bengali texts in reduced dimension using deep feedforward neural network for categorization},
  author={Purkaystha, Bishwajit and Datta, Tapos and Islam, Md Saiful and others},
  booktitle={2018 21st International Conference of Computer and Information Technology (ICCIT)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}


@article{lundberg2017unified,
  title={A unified approach to interpreting model predictions},
  author={Lundberg, Scott M and Lee, Su-In},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{alam2018bard,
  title={Bard: Bangla article classification using a new comprehensive dataset},
  author={Alam, Md Tanvir and Islam, Md Mofijul},
  booktitle={2018 International Conference on Bangla Speech and Language Processing (ICBSLP)},
  pages={1--5},
  year={2018},
  organization={IEEE}
}

@article{minaee2021deep,
  title={Deep learning--based text classification: a comprehensive review},
  author={Minaee, Shervin and Kalchbrenner, Nal and Cambria, Erik and Nikzad, Narjes and Chenaghlu, Meysam and Gao, Jianfeng},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={3},
  pages={1--40},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@inproceedings{al2018bangla,
  title={Bangla content categorization using text based supervised learning methods},
  author={Al Mostakim, Sadek and Ehsan, Faiza and Hasan, Syeda Mahdiea and Islam, Sadia and Shatabda, Swakkhar},
  booktitle={2018 International Conference on Bangla Speech and Language Processing (ICBSLP)},
  pages={1--6},
  year={2018},
  organization={IEEE}
}

@article{lopez2013insight,
  title={An insight into classification with imbalanced data: Empirical results and current trends on using data intrinsic characteristics},
  author={L{\'o}pez, Victoria and Fern{\'a}ndez, Alberto and Garc{\'\i}a, Salvador and Palade, Vasile and Herrera, Francisco},
  journal={Information sciences},
  volume={250},
  pages={113--141},
  year={2013},
  publisher={Elsevier}
}

@article{padurariu2019dealing,
  title={Dealing with data imbalance in text classification},
  author={Padurariu, Cristian and Breaban, Mihaela Elena},
  journal={Procedia Computer Science},
  volume={159},
  pages={736--745},
  year={2019},
  publisher={Elsevier}
}

@article{islam2017comparative,
  title={A comparative study on different types of approaches to Bengali document categorization},
  author={Islam, Md and Jubayer, Fazla Elahi Md and Ahmed, Syed Ikhtiar and others},
  journal={arXiv preprint arXiv:1701.08694},
  year={2017}
}

@inproceedings{joachims1998text,
  title={Text categorization with support vector machines: Learning with many relevant features},
  author={Joachims, Thorsten},
  booktitle={European conference on machine learning},
  pages={137--142},
  year={1998},
  organization={Springer}
}

@inproceedings{chowdhury2022bangla,
  title={Bangla news classification using GloVe vectorization, LSTM, and CNN},
  author={Chowdhury, Pallab and Eumi, Ettilla Mohiuddin and Sarkar, Ovi and Ahamed, Md and others},
  booktitle={Proceedings of the International Conference on Big Data, IoT, and Machine Learning},
  pages={723--731},
  year={2022},
  organization={Springer}
}

@inproceedings{amin2020multiclass,
  title={Multiclass classification for bangla news tags with parallel cnn using word level data augmentation},
  author={Amin, Ruhul and Sworna, Nabila Sabrin and Hossain, Nahid},
  booktitle={2020 IEEE Region 10 Symposium (TENSYMP)},
  pages={174--177},
  year={2020},
  organization={IEEE}
}

@incollection{hasib2022imbalanced,
  title={Imbalanced Data Classification Using Hybrid Under-Sampling with Cost-Sensitive Learning Method},
  author={Hasib, Khan Md and Showrov, Md and Hossain, Imran and Al Mahmud, Jubayer and Mithu, Kamruzzaman},
  booktitle={Edge Analytics},
  pages={423--435},
  year={2022},
  publisher={Springer}
}

@article{kumari2022supervised,
  title={Supervised link prediction using structured-based feature extraction in social network},
  author={Kumari, Anisha and Behera, Ranjan Kumar and Sahoo, Kshira Sagar and Nayyar, Anand and Kumar Luhach, Ashish and Prakash Sahoo, Satya},
  journal={Concurrency and Computation: practice and Experience},
  volume={34},
  number={13},
  pages={e5839},
  year={2022},
  publisher={Wiley Online Library}
}

@article {10.3844/jcssp.2022.1170.1178,
article_type = {journal},
title = {Emotion Recognition from Microblog Managing Emoticon with Text and Classifying using 1D CNN},
author = {Habib, Md. Ahsan and Akhand, M. A. H. and Kamal, Md. Abdus Samad},
volume = {18},
number = {12},
year = {2022},
month = {Dec},
pages = {1170-1178},
doi = {10.3844/jcssp.2022.1170.1178},
url = {https://thescipub.com/abstract/jcssp.2022.1170.1178},
abstract = {Microblog, an online-based broadcast medium, is a widely used forum for people to share their thoughts and opinions. Recently, Emotion Recognition (ER) from microblogs is an inspiring research topic in diverse areas. In the machine learning domain, automatic emotion recognition from microblogs is a challenging task, especially, for better outcomes considering diverse content. Emoticon becomes very common in the text of microblogs as it reinforces the meaning of content. This study proposes an emotion recognition scheme considering both the texts and emoticons from microblog data. Emoticons are considered unique expressions of the users&#039; emotions and can be changed by the proper emotional words. The succession of emoticons appearing in the microblog data is preserved and a 1D Convolutional Neural Network (CNN) is employed for emotion classification. The experimental result shows that the proposed emotion recognition scheme outperforms the other existing methods while tested on Twitter data.},
journal = {Journal of Computer Science},
publisher = {Science Publications}
}

@inproceedings{dhar2022transformer,
  title={Transformer Deep Learning Model for Bangla--English Machine Translation},
  author={Dhar, Argha Chandra and Roy, Arna and Habib, Md and Akhand, MAH and Siddique, N and others},
  booktitle={Proceedings of 2nd International Conference on Artificial Intelligence: Advances and Applications},
  pages={255--265},
  year={2022},
  organization={Springer}
}

@article{islam2021recognition,
  title={Recognition of Emotion from Emoticon with Text in Microblog Using LSTM},
  author={Islam, Juyana and Akhand, MAH and Habib, Md Ahsan and Kamal, Md Abdus Samad and Siddique, Nazmul},
  journal={Advances in Science, Technology and Engineering Systems Journal},
  volume={6},
  number={3},
  pages={347--354},
  year={2021}
}

@article{devi2022irko,
  title={IRKO: an improved Runge-Kutta optimization algorithm for global optimization problems},
  author={Devi, R Manjula and Premkumar, M and Jangir, Pradeep and Elkotb, Mohamed Abdelghany and Elavarasan, Rajvikram Madurai and Nisar, Kottakkaran Sooppy},
  journal={CMC-COMPUTERS MATERIALS \& CONTINUA},
  volume={70},
  number={3},
  pages={4803--4827},
  year={2022},
  publisher={TECH SCIENCE PRESS 871 CORONADO CENTER DR, SUTE 200, HENDERSON, NV 89052 USA}
}

@article{gupta2021partition,
  title={A partition cum unification based genetic-firefly algorithm for single objective optimization},
  author={Gupta, Dhrubajyoti and Dhar, Ananda Rabi and Roy, Shibendu Shekhar},
  journal={S{\=a}dhan{\=a}},
  volume={46},
  number={3},
  pages={1--31},
  year={2021},
  publisher={Springer}
}

@article{ghasemi2022circulatory,
  title={Circulatory System Based Optimization (CSBO): An expert multilevel biologically inspired meta-heuristic algorithm},
  author={Ghasemi, Mojtaba and Akbari, Mohammad-Amin and Jun, Changhyun and Bateni, Sayed M and Zare, Mohsen and Zahedi, Amir and Pai, Hao-Ting and Band, Shahab S and Moslehpour, Massoud and Chau, Kwok-Wing},
  journal={Engineering Applications of Computational Fluid Mechanics},
  volume={16},
  number={1},
  pages={1483--1525},
  year={2022},
  publisher={Taylor \& Francis}
}

@article{zhao2021decomposition,
  title={A decomposition and multi-objective evolutionary optimization model for suspended sediment load prediction in rivers},
  author={Zhao, Nannan and Ghaemi, Alireza and Wu, Chengwen and Band, Shahab S and Chau, Kwok-Wing and Zaguia, Atef and Mafarja, Majdi and Mosavi, Amir H},
  journal={Engineering Applications of Computational Fluid Mechanics},
  volume={15},
  number={1},
  pages={1811--1829},
  year={2021},
  publisher={Taylor \& Francis}
}

@article{wang2020yin,
  title={Yin-Yang firefly algorithm based on dimensionally Cauchy mutation},
  author={Wang, Wen-chuan and Xu, Lei and Chau, Kwok-wing and Xu, Dong-mei},
  journal={Expert Systems with Applications},
  volume={150},
  pages={113216},
  year={2020},
  publisher={Elsevier}
}

@article{sammen2020enhanced,
  title={Enhanced artificial neural network with Harris hawks optimization for predicting scour depth downstream of ski-jump spillway},
  author={Sammen, Saad Sh and Ghorbani, Mohammad Ali and Malik, Anurag and Tikhamarine, Yazid and AmirRahmani, Mohammad and Al-Ansari, Nadhir and Chau, Kwok-Wing},
  journal={Applied Sciences},
  volume={10},
  number={15},
  pages={5160},
  year={2020},
  publisher={MDPI}
}

@article{kumar2022generative,
  title={Generative adversarial network (GAN) and enhanced root mean square error (ERMSE): deep learning for stock price movement prediction},
  author={Kumar, Ashish and Alsadoon, Abeer and Prasad, PWC and Abdullah, Salma and Rashid, Tarik A and Pham, Duong Thu Hang and Nguyen, Tran Quoc Vinh},
  journal={Multimedia Tools and Applications},
  volume={81},
  number={3},
  pages={3995--4013},
  year={2022},
  publisher={Springer}
}

@article{hong2022screening,
  title={Screening ideas in the early stages of technology development: A word2vec and convolutional neural network approach},
  author={Hong, Suckwon and Kim, Juram and Woo, Han-Gyun and Kim, Young-Choon and Lee, Changyong},
  journal={Technovation},
  volume={112},
  pages={102407},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{chowdhury2022bangla,
  title={Bangla news classification using GloVe vectorization, LSTM, and CNN},
  author={Chowdhury, Pallab and Eumi, Ettilla Mohiuddin and Sarkar, Ovi and Ahamed, Md and others},
  booktitle={Proceedings of the International Conference on Big Data, IoT, and Machine Learning},
  pages={723--731},
  year={2022},
  organization={Springer}
}

@article{ali2021multi,
  title={Multi-level Kronecker Convolutional Neural Network (ML-KCNN) for Glioma Segmentation from Multi-modal MRI Volumetric Data},
  author={Ali, Muhammad Junaid and Raza, Basit and Shahid, Ahmad Raza},
  journal={Journal of Digital Imaging},
  volume={34},
  number={4},
  pages={905--921},
  year={2021},
  publisher={Springer}
}

@inproceedings{chakraborty2022ternary,
  title={A Ternary Sentiment Classification of Bangla Text Data using Support Vector Machine and Random Forest Classifier},
  author={Chakraborty, Partha and Nawar, Farah and Chowdhury, Humayra Afrin},
  booktitle={International Conference on Computational Techniques and Applications},
  pages={69--77},
  year={2022},
  organization={Springer}
}

@incollection{ahmed2022bangla,
  title={Bangla Document Categorization Using Deep RNN Model with Attention Mechanism},
  author={Ahmed, Mostaq and Chakraborty, Partha and Choudhury, Tanupriya},
  booktitle={Cyber Intelligence and Information Retrieval},
  pages={137--147},
  year={2022},
  publisher={Springer}
}

@article{ahmed2022dad,
  title={DAD-Net: Classification of Alzheimer’s Disease Using ADASYN Oversampling Technique and Optimized Neural Network},
  author={Ahmed, Gulnaz and Er, Meng Joo and Fareed, Mian Muhammad Sadiq and Zikria, Shahid and Mahmood, Saqib and He, Jiao and Asad, Muhammad and Jilani, Syeda Fizzah and Aslam, Muhammad},
  journal={Molecules},
  volume={27},
  number={20},
  pages={7085},
  year={2022},
  publisher={MDPI}
}

@article{vikram2021accelerated,
  title={Accelerated screening of colloidal nanocrystals using artificial neural network-assisted autonomous flow reactor technology},
  author={Vikram, Ajit and Brudnak, Ken and Zahid, Arwa and Shim, Moonsub and Kenis, Paul JA},
  journal={Nanoscale},
  volume={13},
  number={40},
  pages={17028--17039},
  year={2021},
  publisher={Royal Society of Chemistry}
}
